Neuron ranking -- an informed way to condense convolutional neural networks architecture

Convolutional neural networks (CNNs) in recent years have made a dramatic impact in science, technology and industry, yet the theoretical mechanism of CNN architecture design remains surprisingly vague. The CNN neurons, including its distinctive element, convolutional filters, are known to be learnable features, yet their individual role in producing the output is rather unclear. The thesis of this work is that not all neurons are equally important and some of them contain more useful information to perform a given task . Consequently, we quantify the significance of each filter and rank its importance in describing input to produce the desired output. This work presents two different methods: (1) a game theoretical approach based on Shapley value which computes the marginal contribution of each filter; and (2) a probabilistic approach based on what-we-call, the Importance switch using variational inference. Strikingly, these two vastly different methods produce similar experimental results, confirming the general theory that some of the filters are inherently more important that the others. The learned ranks can be readily useable for network compression and interpretability.

==> toaddlater.tex <==
To summarize, the metric allows to compute the individual cost for each feature given the information about all the coalitions. Given the information about each feature, we may establish a ranking of features ranking them from the feature that carries the largest cost, and therefore  contains the most crucial information about the input which is the most helpful in the further inf, deeming it most important. In a similar fashion, least important nodes can be identified whose removal from the network will hardly cost the network. 


In the convolutional neural network (CNN), the layerwise structure of the network produces a hierarchy of features. As each layer forms a separate entity in the hierarchy, we investigate separately the features in each layer and select the features which are deemed most important for a particular machine learning task.



%BACKUP

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum1_epoch-1.png}
  \end{minipage}
  %\hfill
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum8_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum3_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum7_epoch-1.png}
  \end{minipage}
  \hfill
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum5_epoch-1.png}
  \end{minipage}
  \hfill
    \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum0_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum7_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum5_epoch-1.png}
  \end{minipage}
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum6_epoch-1.png}
  \end{minipage}\hfill
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum8_epoch-1.png}
  \end{minipage}
  
    \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum1_epoch-1.png}
  \end{minipage}
  %\hfill
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum8_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum7_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum3_epoch-1.png}
  \end{minipage}
  \hfill
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum5_epoch-1.png}
  \end{minipage}
  \hfill
    \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum0_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum7_epoch-1.png}
  \end{minipage}
  \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum5_epoch-1.png}
  \end{minipage}
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum6_epoch-1.png}
  \end{minipage}\hfill
   \begin{minipage}[b]{0.085\textwidth}
    \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum8_epoch-1.png}
  \end{minipage}
  \caption{Visualization of four important and one unimportant feature maps produced by Shapley value and importance switches algorithms as given in Table 2. MNIST:  Filters 1,8,3,7, FashionMNIST 0,7,5,6. Notice the complementary nature of important features MNIST: (1,3), FashionMNIST (0,7) and reinforcing features: MNIST (1,8), FashionMNIST (7,5). The unimportant features are jagged and lack concrete focus.}
\end{figure}

%%%%%%compression

\begin{table}[]
% \vspace{-0.4em}
\label{tab:table_comp}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        Method & Architecture & FLOPs & Params & Error\\
  	\hline
          \textbf{FR (proposed)} &\textbf{5-7-45-20}& \textbf{125K} & \textbf{20K} & \textbf{1.08\%} \\
          RDP &4-7-110-66& 125K & 20K & 1.0\%} \\
        
          BC-GNJ & 8-13-88-13&  307K & 22K & 1.0\%\\
          BC-GHS & 5-10-76-16& 169K & \textbf{15K} & 1.0\%\\
          FDOO(100K) & 2-7-112-478& \textbf{119K} & 66K & 1.1\%\\
          FDOO(200K) & 3-8-128-499& 163K & 81K & 1.0\% \\
        
           GL & 3-12-192-500& 236K & 134K & 1.0\% \\
           GD & 7-13-208-16& 298K & 49K & 1.1\% \\
            SBP & 3-18-284-283& 295K & 164K & \textbf{0.9\%} \\
        \hline
        \textbf{FR (proposed)} & \textbf{34-34-68-68-75-106-101-92-102-92-92-67-67-62-62}&  &  & 8.6\%\\
         BC-GNJ & 63-64-128-128-245-155-63-26-24-20-14-12-11-11-15&  &  & 8.3\%\\
          BC-GHS & 51-62-125-128-228-129-38-13-9-6-5-6-6-6-20&  &  & 8.3\%\\
          \hline
    
    \end{tabular}
    % \vspace{-0.6em}
    \caption{The structured pruning of LeNet-5-Caffe with the original architecture 20-50-800-500. We benchmark our method against BC-GNJ, Bayesian Compression-Group HorseShoe(BC-GHS)~\cite{louizos2017bayesian}, FDOO~\cite{tang2018flops}, Generalized Dropout(GD)~\cite{srinivas2015data}, Group Lasso(GL)~\cite{wen2016learning}, 
    Structured Bayesian Pruning(SBP)~\cite{neklyudov2017structured}.
    }
\vspace{-1em}
\end{table}




% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum1_epoch-1.png}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum8_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum7_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum4_epoch-1.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch1_filternum5_epoch-1.png}
%   \end{minipage}
%   \hfill
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum0_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum7_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum6_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum5_epoch-1.png}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch0_filternum8_epoch-1.png}
%   \end{minipage}
  
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum0_epoch-1.png}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum0_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum7_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum5_epoch-1.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/mnist/conv1_batch0_filternum9_epoch-1.png}
%   \end{minipage}
%   \hfill
%   %FASHION SWITCHES
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum0_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum7_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum5_epoch-1.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum9_epoch-1.png}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{images/paper_right/fashionmnist/conv1_batch4_filternum8_epoch-1.png}
%   \end{minipage}
%   \caption{Visualization of four important and one unimportant feature maps produced by Shapley value and importance switches algorithms as given in Table 2. MNIST:  Filters 1,8,3,7, FashionMNIST 0,7,5,6. Notice the complementary nature of important features MNIST: (1,3), FashionMNIST (0,7) and reinforcing features: MNIST (1,8), FashionMNIST (7,5). The unimportant features are jagged and lack concrete focus.}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
  
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     %\includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
  
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     %\includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%     \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
% \end{figure}


% spaces matter between minipages
% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}

%   \end{minipage}
%   %\hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
  
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
  
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%   \end{minipage}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%     \caption{Flower one.}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.085\textwidth}
  
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%     \caption{Flower one.}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.085\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%     \caption{Flower one.}
%   \end{minipage}
%   \hfill

% \end{figure}


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{flower1.jpg}
%     \caption{Flower one.}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{flower2.jpg}
%     \caption{Flower two.}
%   \end{minipage}
% \end{figure}


